Query Rewriting On Path Views Without Integrity Constraints

A view with a binding pattern is a parameterised query on a database. Such views are used, e.g., to model Web services. To answer a query on such views, one has to orchestrate the views together in execution plans. The goal is usually to find equivalent rewritings, which deliver precisely the same results as the query on all databases. However, such rewritings are usually possible only in the presence of integrity constraints - and not all databases have such constraints. In this paper, we describe a class of plans that give practical guarantees about their result even if there are no integrity constraints. We provide a characterisation of such plans and a complete and correct algorithm to enumerate them. Finally, we show that our method can find plans on real-world Web Services.

==> images/CIKM2018/dangie-plan-and-database.tex <==
\tikzstyle arrowstyle=[blue,semitransparent,scale=2]
\tikzstyle basiclabel=[draw=none,fill=none,shape=rectangle,inner sep=2pt,scale=.8]
\tikzstyle leftlabel=[basiclabel,anchor=east]
\tikzstyle rightlabel=[basiclabel,anchor=west]
\tikzstyle bottomlabel=[basiclabel,anchor=north]
\tikzstyle toplabel=[basiclabel,anchor=south]

%%%%%%%%%%%%%%%%%
% Define block styles
\definecolor{lightblue}{cmyk}{0.12,0,0,0.15} 
\tikzstyle{block} = [rectangle, draw, fill=white, 
text centered, rounded corners]

\definecolor{darkpastelgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{dartmouthgreen}{rgb}{0.05, 0.5, 0.06}
\definecolor{forestgreen}{rgb}{0.0, 0.27, 0.13}
\definecolor{lasallegreen}{rgb}{0.03, 0.47, 0.19}


\tikzstyle{headvar} = [rectangle, draw, fill=lightblue!70,
text centered, rounded corners]    
\tikzstyle{labelcase} = [rectangle,    text centered]
\tikzstyle{background}=[rectangle,   fill=lightblue!70,
inner sep=0.2cm,
rounded corners=5mm]

\tikzstyle{line} = [draw, -latex']
\tikzstyle{linenoarrow} = [draw]
\tikzstyle{invisibleline} = [-latex',sloped]
\tikzstyle{dashedline} = [draw, dashed]
\tikzstyle{inputtar} = [rectangle, draw, fill=lightblue!70, 
text centered, rounded corners]

\tikzstyle{inputvar} = [rectangle, draw=red,  fill=red!30,
text centered, rounded corners]

%\includegraphics[width=\columnwidth]{./fig/cases-1.pdf}
\begin{tikzpicture}[scale=0.9, transform shape]



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%database
\node [block] (p1) {\textit{Anna}};
\node [block] (c1) at ($(p1)+(-2.8cm,0cm)$) {\textit{The Guardian}};
\node [block] (tel1) at ($(p1)+(+2.2cm,0cm)$) {\textit{01.22.33.44}};

\path [line] (p1) --node [above,align=center] {{\textit{worksAt}} } (c1);
\path [line] (p1) --node [above,align=center] {{\textit{phone}} } (tel1);



\node [block] (dep1) at ($(p1)+(0,-2.5cm)$){\textit{Economy Section}};
\path [line] (p1) --node [sloped,above, align=center] {{\textit{headOf}} } (dep1);


%function getAlbumDetails
\coordinate (xb) at   ($(p1) + (-0.5cm,-0.4cm) $);
\coordinate (yb) at   ($(c1) +  (+0cm,-0.4cm) $);
\coordinate (zb) at   ($(dep1) +  (-0.5cm,+0.4cm) $);
\draw [blue]    (yb) to (xb);
\draw [->,blue]    (xb) to (zb);
\node [labelcase,blue] (lf2) at   ($0.5*(xb) + 0.5*(yb) + (0cm,-0.18cm)$) {\textit{getSection}};

%function getAlbumDetails
\coordinate (xc) at   ($(p1) + (+0.5cm,-0.4cm) $);
\coordinate (yc) at   ($(tel1) +  (+0cm,-0.4cm) $);
\coordinate (zc) at   ($(dep1) +  (+0.5cm,+0.4cm) $);
\draw [->,blue]    (xc) to (yc);
\draw [blue]    (xc) to (zc);
\node [labelcase,blue] (lf3) at   ($0.5*(xc) + 0.5*(yc) + (0cm,-0.18cm)$) {\textit{getPhone}};


\node [inputvar] (p2) at ($(c1)+(-3cm,0cm)$) {\textit{Johnson}};
\path [line] (p2) --node [above,align=center] {{\textit{worksAt}} } (c1);
%function getAlbum
\coordinate (p2up) at   ($(p2) + (+0.4cm,-0.4cm) $); 
\coordinate (c1up) at   ($(c1) + (-0.2cm,-0.4cm) $); 
\draw [blue,->]     (p2up) to  (c1up);
\node [labelcase,blue] (lf1) at   ($0.5*(p2up) + 0.5*(c1up) + (0,-0.18cm)$) {\textit{getCompany}};

\node [inputvar] (tel2) at ($(p2)+(-1.9cm,0cm)$) {?};
\path [line,red] (p2) --node [above,align=center] {{\textit{phone}} } (tel2);

\end{tikzpicture}


==> images/CIKM2018/dangie-plan.tex <==
\tikzstyle arrowstyle=[blue,semitransparent,scale=2]
\tikzstyle basiclabel=[draw=none,fill=none,shape=rectangle,inner sep=2pt,scale=.8]
\tikzstyle leftlabel=[basiclabel,anchor=east]
\tikzstyle rightlabel=[basiclabel,anchor=west]
\tikzstyle bottomlabel=[basiclabel,anchor=north]
\tikzstyle toplabel=[basiclabel,anchor=south]

%%%%%%%%%%%%%%%%%
% Define block styles
\definecolor{lightblue}{cmyk}{0.12,0,0,0.15} 
\tikzstyle{block} = [rectangle, draw, fill=white, 
text centered, rounded corners]

\definecolor{darkpastelgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{dartmouthgreen}{rgb}{0.05, 0.5, 0.06}
\definecolor{forestgreen}{rgb}{0.0, 0.27, 0.13}
\definecolor{lasallegreen}{rgb}{0.03, 0.47, 0.19}


\tikzstyle{headvar} = [rectangle, draw, fill=lightblue!70,
text centered, rounded corners]    
\tikzstyle{labelcase} = [rectangle,    text centered]
\tikzstyle{background}=[rectangle,   fill=lightblue!70,
inner sep=0.2cm,
rounded corners=5mm]

\tikzstyle{line} = [draw, -latex']
\tikzstyle{linenoarrow} = [draw]
\tikzstyle{invisibleline} = [-latex',sloped]
\tikzstyle{dashedline} = [draw, dashed]
\tikzstyle{inputtar} = [rectangle, draw, fill=lightblue!70, 
text centered, rounded corners]

\tikzstyle{inputvar} = [rectangle, draw=red,  fill=red!30,
text centered, rounded corners]

%\includegraphics[width=\columnwidth]{./fig/cases-1.pdf}
\begin{tikzpicture}[scale=0.9, transform shape]



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%database
\node [inputvar] (f1p1) {\textit{Anna}};
\node [block] (f1c1) at ($(f1p1)+(-3cm,0cm)$) {\textit{The Guardian}};
\node [block] (f1tel1) at ($(f1p1)+(+2.3cm,0cm)$) {\textit{01.22.33.44}};

\path [line] (f1p1) --node [above,align=center] {{\textit{worksAt}} } (f1c1);
\path [line,red] (f1p1) --node [above,align=center] {{\textit{phone}} } (f1tel1);



\node [block] (f1dep1) at ($(f1p1)+(0,-2.2cm)$){\textit{Economy Section}};
\path [line] (f1p1) --node [sloped,above, align=center] {{\textit{headOf}} } (f1dep1);


%function getAlbumDetails
\coordinate (f1xb) at   ($(f1p1) + (-0.5cm,-0.4cm) $);
\coordinate (f1yb) at   ($(f1c1) +  (+0cm,-0.4cm) $);
\coordinate (f1zb) at   ($(f1dep1) +  (-0.5cm,+0.4cm) $);
\draw [blue]    (f1yb) to (f1xb);
\draw [->,blue]    (f1xb) to (f1zb);
\node [labelcase,blue] (f1lf2) at   ($0.5*(f1xb) + 0.5*(f1yb) + (0cm,-0.18cm)$) {\textit{getSection}};

%function getAlbumDetails
\coordinate (f1xc) at   ($(f1p1) + (+0.5cm,-0.4cm) $);
\coordinate (f1yc) at   ($(f1tel1) +  (+0cm,-0.4cm) $);
\coordinate (f1zc) at   ($(f1dep1) +  (+0.5cm,+0.4cm) $);
\draw [->,blue]    (f1xc) to (f1yc);
\draw [blue]    (f1xc) to (f1zc);
\node [labelcase,blue] (f1lf3) at   ($0.5*(f1xc) + 0.5*(f1yc) + (0cm,-0.18cm)$) {\textit{getPhone}};


%function getAlbum
\coordinate (f1p1up) at   ($(f1p1) + (+0.4cm,+0.4cm) $); 
\coordinate (f1c1up) at   ($(f1c1) + (-0.2cm,+0.4cm) $); 
\draw [blue,->]     (f1p1up) to  (f1c1up);
\node [labelcase,blue] (f1lf1) at   ($0.5*(f1p1up) + 0.5*(f1c1up) + (0,+0.2cm)$) {\textit{getCompany}};

\end{tikzpicture}


==> images/CIKM2018/fig-album-producer.tex <==
\tikzstyle arrowstyle=[blue,semitransparent,scale=2]
\tikzstyle basiclabel=[draw=none,fill=none,shape=rectangle,inner sep=2pt,scale=.8]
\tikzstyle leftlabel=[basiclabel,anchor=east]
\tikzstyle rightlabel=[basiclabel,anchor=west]
\tikzstyle bottomlabel=[basiclabel,anchor=north]
\tikzstyle toplabel=[basiclabel,anchor=south]

%%%%%%%%%%%%%%%%%
% Define block styles
\definecolor{lightblue}{cmyk}{0.12,0,0,0.15} 
\tikzstyle{block} = [rectangle, draw, fill=white, 
     text centered, rounded corners]
\tikzstyle{labelcase} = [rectangle,    text centered]
\tikzstyle{background}=[rectangle,   fill=lightblue!70,
                                                inner sep=0.2cm,
                                                rounded corners=5mm]

\tikzstyle{line} = [draw, -latex']
\tikzstyle{dashedline} = [draw, dashed]
%line width=0.3mm,
\tikzstyle{inputvar} = [rectangle, draw=red,  fill=red!30,
     text centered, rounded corners]



%\includegraphics[width=\columnwidth]{./fig/cases-1.pdf}
\begin{tikzpicture}[scale=0.9, transform shape]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% getProducer
\node [inputvar] (x) {\underline{$s$}};
\node [block, right of=x, node distance=1.8cm, align= flush center] (y) {$a$};
\path [line] (x) --node [above,align=center] {{\em onAlbum}} (y);
\coordinate (ix) at   ($(x) + (-0.7cm,0) $); 
\node [block, right of=y, node distance=2.1cm, align= flush center] (z) {$p$};
\path [line] (z) --node [above,align=center] {{\em producer}} (y);


\node [labelcase] (fgGC) at   ($0.5*(y) + 0.5*(z) + (-1cm,-0.8cm) $) {{\em getProducer$(\underline{s},a,p)$}};



% getProducedAlbum
\node [inputvar, right of=z, node distance=4cm] (xGF) {\underline{$p$}};
\node [block, left of=xGF, node distance=2.1cm, align= flush center] (yGF) {$a$};
\path [line] (yGF) --node [above,align=center] {{\em producer}} (xGF);

\coordinate (ixGF) at   ($(xGF) + (0.7cm,0) $); 
\node [labelcase] (fGF) at   ($0.5*(yGF) + 0.5*(xGF) - (0,0.8cm)$) {{\em getProducedAlbum$(\underline{p},a)$}};


% Query
%\node [block, below of=x, node distance=2cm] (qg) {{$m$}};
%\node [block, right of=qg, node distance=2cm, align= flush center] (qn) {{\em Jailhouse}};
%\path [line] (qg) --node [above,align=center] {{\em sang}} (qn);
%\node [labelcase] (qQuery) at   ($(qg) - (-0.6,+0.8cm)$) {{\em Query }};


\end{tikzpicture}

